Robust Model Selection and Nearly-Proper Learning for GMMs

In learning theory, a standard assumption is that the data is generated from a finite mixture model. But what happens when the number of components is not known in advance? The problem of estimating the number of components, also called model selection, is important in its own right but there are essentially no known efficient algorithms with provable guarantees let alone ones that can tolerate adversarial corruptions. In this work, we study the problem of robust model selection for univariate Gaussian mixture models (GMMs). Given $\textsf{poly}(k/\epsilon)$ samples from a distribution that is $\epsilon$-close in TV distance to a GMM with $k$ components, we can construct a GMM with $\widetilde{O}(k)$ components that approximates the distribution to within $\widetilde{O}(\epsilon)$ in $\textsf{poly}(k/\epsilon)$ time. Thus we are able to approximately determine the minimum number of components needed to fit the distribution within a logarithmic factor. Prior to our work, the only known algorithms for learning arbitrary univariate GMMs either output significantly more than $k$ components (e.g. $k/\epsilon^2$ components for kernel density estimates) or run in time exponential in $k$. Moreover, by adapting our techniques we obtain similar results for reconstructing Fourier-sparse signals.

==> introduction.tex <==
\section{Introduction}

Many works in signal processing and learning theory operate under the assumption that the underlying model is {\em simple}. We will be interested in two particular settings:

\paragraph{Fourier-Sparse Interpolation}

We would like to interpolate a signal based on noisy measurements of it at a few points \cite{chen2016fourier}. In particular, we assume we can measure a signal
$f(t) = \mcl{M}(t) + \eta(t)$
at any point in the interval $[-1, 1]$. Here $\mcl{M}(t)$ is a structured signal that has a $k$-sparse Fourier representation \--- i.e.
$$ \mcl{M}(t) = \sum_{j=1}^k a_j e^{2 \pi i \theta_j t}$$
Furthermore we assume that $\sum_j |a_j| \leq 1$ and each frequency $\theta_j$ is in the interval $[-F, F]$. Finally $\eta(t)$ is noise that we will assume is bounded in $L_2$ norm. The goal is to compute a Fourier-sparse approximation $\widetilde{\mcl{M}}(t)$ that is close to $f(t)$, in the sense that its error is comparable to that of $\mcl{M}(t)$. 

\paragraph{Robustly Learning One-dimensional Gaussian Mixture Models}

We would like to estimate the components of a one-dimensional mixture model from samples. In particular, we are given random samples from a distribution $f$ with the property that it is well-approximated by a Gaussian mixture model with at most $k$ components \--- i.e. we can write
$f(x) = \mathcal{M}(x) + \eta(x)$
where
$$\mathcal{M}(x) = \sum_{i =1}^k w_i G_i(x)$$
and the $w_i$'s are the mixing weights and the $G_i$'s are Gaussians. Moreover $\eta(x)$ is the noise, and we will assume that its $L_1$ norm is at most $2\epsilon$ and that it integrates to zero so that $f(x)$ is a distribution which satisfies $d_{TV}(f, \mathcal{M}) \leq \epsilon$. The goal is to compute an approximation $\widetilde{\mathcal{M}}(x)$ to $f(x)$ that is a GMM and that is $O(\epsilon)$-close in total variation distance. 
\\

Both of these problems exhibit the same structured plus noise decomposition, and share the feature that the structured portion is a sum/mixture of at most $k$ simple building blocks. These problems have been intensively investigated. Many existing results focus on the {\em unique recovery problem}, where the goal is not merely to compete with the best $k$-sparse approximation but to uniquely recover its parameters (when the noise is sufficiently small, or even zero). The difficulty is for both of these problems you usually need to make a separation assumption to do this. In particular, Moitra \cite{moitra2015super} showed that for Fourier-sparse interpolation if the minimum separation between the frequencies is beneath some critical threshold, you need the noise to be exponentially small even to approximate the constituent frequencies. See also \cite{chen2020algorithmic}. Similarly, Moitra and Valiant \cite{moitra2010settling} showed that for Gaussian mixture models you need the number of samples to grow exponentially in $k$ to estimate the mixture on a component-by-component basis. 

But what happens if we do not impose a separation condition? There are exponential time algorithms for both Fourier-sparse interpolation \cite{chen2019active, avron2019universal} and learning Gaussian mixture models \cite{daskalakis2014faster, acharya2014near} that perform a grid search over the parameters. Alternatively we can relax the requirement that we output a model with exactly $k$ frequencies/components polynomial time algorithms are known. Chen, Kane, Price and Song \cite{chen2016fourier} studied Fourier-sparse interpolation without a frequency gap and showed how to construct an approximation $\widetilde{\mcl{M}}(t)$ that satisfies
$$\|f(t) - \widetilde{\mcl{M}}(t)\|_2 \leq \| \eta(t) \|_2 + \eps \|\mcl{M}(t)\|_2$$
where the $L_2$ norm is taken over the interval $[-1, 1]$. Their algorithm works for any $\eps > 0$ and uses $\mbox{poly}(k, \log 1/\eps) \log F$ measurements. Moreover the $\widetilde{\mcl{M}}(t)$ that they output is $\mbox{poly}(k, \log 1/\eps)$-Fourier sparse. For Gaussian mixture models, kernel density estimators output an estimate $\widetilde{\mathcal{M}}$ with $O(k/\epsilon^2)$ components that satisfies
$$d_{\TV}(f, \widetilde{\mathcal{M}}) = O(\epsilon)$$
There are also approaches based on piece-wise polynomial approximation \cite{chan2013efficient, acharya2017sample}.
For us, the key point is that these estimators have many more frequencies/components than we started off with. Our main question is:

\begin{question}
Can we find sparser approximations for Fourier-sparse interpolation and learning in Gaussian mixture models?
\end{question}

\noindent An important motivation for studying this question comes from {\em model selection}. In particular:

\begin{question}
What happens when we don't know $k$ in advance?
\end{question}

In fact, in many scientific applications where we expect our signals to be Fourier-sparse or where we expect our distribution to be well-approximated by a Gaussian mixture model, choosing the number of frequencies/components is the most important issue. Consider the motivation given by Chen et al. \cite{chen2004testing}: In genetics, there are many situations where we have a continuous-valued trait that we can measure across a population and we want to understand its genetic basis. In fact it is often not clear whether the underlying genetic mechanism is simple or complex \--- i.e. is it controlled by just a few genes or are there many more genes waiting to be discovered that each have a small effect on the trait? These problems are often modeled by one-dimensional Gaussian mixture models \cite{chen2004testing}. 


In summary, when we model a signal as Fourier-sparse or a distribution as being well-approximated by a mixture model, the frequencies/components usually represent some features of a natural process that we would like to extract and understand from data. Determining the number of components amounts to deciding whether we already have an accurate scientific model, or if there is more complexity to be discovered. So what can we say algorithmically about model selection? We could always run our interpolation/learning algorithms for different values of $k$ and decide afterwards which one among them is a better balance of fit vs. complexity. However therein lies the problem: The models that existing algorithms output are much more complex than what we started out with. So we don't know whether the fact that we found many frequencies/components is because no simple model fits our data, or because it's a failing of our algorithm. 

Model selection, particularly choosing the number of components in a Gaussian mixture model, has been intensively studied in statistics for over fifty years \cite{neyman1966use}. From a statistical perspective what makes the problem challenging is that standard analysis of the likelihood ratio test breaks down because of lack of regularity and non-identifiability \cite{hartigan1985failure}. Despite many attempts \cite{ghosh1984asymptotic, lo2001testing, huang2017model} and rejoinders \cite{jeffries2003note}, even understanding the asymptotic distribution of the likelihood ratio statistics has been described as a long-standing challenge in the field \cite{kasahara2015testing}. In fact the algorithmic problems run even deeper: Even if we could analyze the likelihood ratio test, ultimately we would need efficient algorithms for computing it and non-asymptotic guarantees. Nevertheless it turns out we will be able to solve an approximate (and robust) version of model selection as an immediate by-product of algorithms. For example:

\begin{question}
Can we test whether a given distribution is close to a Gaussian mixture model with $k$ components, or far from every such model with at most $k' = \widetilde{O}(k)$ components?
\end{question}

Despite a long line of work on the problem of learning a Gaussian mixture model, the only existing guarantees for this problem either:
\begin{enumerate}
    \item[(1)] Need to assume some strong separation condition on the components, e.g. so that they are clusterable
    \item[(2)] Work by first solving the parameter learning problem \cite{moitra2010settling}, in which case we need an exponential in $k$ number of samples even information-theoretically
    \item[(3)] Perform a grid search \cite{daskalakis2014faster, acharya2014near} or solve a system of polynomial equations \cite{li2017robust}, which runs in time exponential in $k$
    \item[(4)] Improperly learn an approximation, e.g. through piece-wise polynomial approximations \cite{chan2013efficient, acharya2017sample}. In such approximations, we can bound the number of pieces based on $k$ and the target accuracy $\epsilon$. However the number of pieces can always be much smaller, in which case we cannot directly use the output of the algorithm to bound the number of components. 
\end{enumerate}
In contrast, our algorithms work without any separation condition and run in polynomial time by slightly relaxing the number of components. We also obtain similar results for model selection in the context of Fourier-sparse interpolation. We remark that the model selection problem we study is conceptually related to tolerant property testing \cite{parnas2006tolerant}. In particular, there is a natural parallel to recent work on relaxed tolerant testing for juntas \cite{diakonikolas2007testing, iyer2021junta} where we would like to distinguish between functions that are $\gamma$-close to $k$-juntas, or $\gamma+\epsilon$-far from every $k' = O(k/\epsilon^2)$-junta through query access. 



\subsection{Our Results and Techniques}

Our first main result is an improved algorithm for Fourier-sparse interpolation. Throughout this paper, for any function $f$, we will use $\widehat{f}$ to denote the Fourier transform of $f$. 

\begin{theorem}\label{thm:fourier-main}
Let $f$ be a function defined on $[-1,1]$ and assume we are given query access to $f$.  Let $\mcl{M}$ be a function that is $k$-Fourier-sparse, has $\norm{\wh{\mcl{M}}}_1 \leq 1$, and has frequencies in the interval $[-F, F]$.  Then for any desired accuracy $\eps > 0$ and constant $c > 0$, in $\poly(k, \log 1/\eps)  \log F  $ queries and $\poly(k /c , \log 1/  \eps)  \log^2 F$ time, we can output a function $\wt{\mcl{M}}$ such that with probability $1 - 2^{-\Omega(k)}$,
\begin{enumerate}
    \item $\wt{\mcl{M}}$ is $k \poly( 1/c, \log k/\eps)$-Fourier sparse with $\norm{\wh{\wt{\mcl{M}}}}_1 \leq k \poly( 1/c, \log k/\eps )$
    \item 
    \[
    \int_{-1 + c}^{1 - c} |\wt{\mcl{M}} - f|^2 \leq  \poly(\log k/(\eps c))\left(\eps^2 + \int_{-1}^1 |f - \mcl{M}|^2 \right) \,.
    \]
\end{enumerate}
\end{theorem}
\begin{remark}
Note the constraints $\norm{\wh{\mcl{M}}}_1 $ and $\norm{\wh{\wt{\mcl{M}}}}_1$ translate into bounds on the sizes of the coefficients of the exponentials in $\mcl{M}$ and $\wt{\mcl{M}}$ respectively. 
\end{remark}

Compared to the results of Chen, Kane, Price and Song \cite{chen2016fourier}, the main differences are that we output a $\widetilde{O}(k)$-Fourier sparse approximation, which is optimal up to polylogarithmic factors. However we can only bound the error on the interval $[-1+c, 1-c]$ for any $c > 0$, for technical reasons. The number of measurements is the same because, in fact, we are able to directly sparsify the output of their algorithm, again invoking the assumption that it is close to a $k$-Fourier sparse signal. 

We obtain the same sort of improvement for fitting a Gaussian mixture model:

\begin{theorem}\label{thm:main-gmm}
Let $\mcl{M} = w_1 G_1 + \dots + w_k G_k$ be an unknown mixture of Gaussians.  Let $k, \eps > 0$ be parameters.  Assume that we are given samples from a distribution $f$ with $d_{\TV}(\mcl{M}, f) \leq \eps$.  Then given $\wt{O}(k /\eps^2)$ samples, there is an algorithm that runs in $\poly(k /\eps)$ time and with probability $0.9$ (over the random samples), outputs a mixture of $\wt{O}(k)$ Gaussians,  $\wt{\mcl{M}}$, such that 
\[
d_{\TV}(\wt{\mcl{M}}, f ) \leq \wt{O}(\eps) \,. 
\]
\end{theorem}

Earlier methods get an approximation with $O(k/\epsilon^2)$ components, which is particularly bad for small values of $\epsilon$. Other algorithms run in exponential in $k$ time. Again, we can take a weak estimator such as a kernel density estimator or a piece-wise polynomial approximation and find a sparse approximation to it, under the assumption that there is one. We remark that in high-dimensions this is already what goes wrong: There is evidence in the form of statistical query lower bounds that approximating a Gaussian mixture model with $k$ components requires exponential time \cite{diakonikolas2017statistical}. 

We take a parallel approach to both of these problems. First, we study the well-conditioned case, where all the frequencies/components are close to each other. These are the hard cases for unique recovery. By reasoning about the Taylor expansion, we show that in the well-conditioned case $O(\log 1/\epsilon)$ terms suffice to get an $O(\epsilon)$-approximation. The key idea is that this structural result allows us to map the building blocks (i.e. complex exponentials/Gaussians) into $O(\log 1/\epsilon)$ dimensional vectors. From there a straightforward application of Caratheodory's theorem tell us that any well-conditioned signal/mixture always has a $O(\log 1/\epsilon)$-sparse $O(\epsilon)$-approximation. Moreover we can make these arguments constructive. In the case of Fourier-sparse interpolation, we show that we can obliviously choose a set of frequencies corresponding to the zeros of a Chebyshev polynomial. Finally, we show how to localize any signal/mixture into well-conditioned parts by multiplying by various Gaussians which effectively zero out distant frequencies/components.  To reconstruct the entire signal/mixture from localized parts, we rely on a result where we approximate the indicator function of an interval as a weighted sum of Gaussians. 

Lastly, we give applications to an approximate version of model selection.  More formally, we can hypothesis test to distinguish between a distribution that is $\eps$-close to a mixture of $k$ Gaussians and a distribution that is not $\wt{O}(\eps)$-close to a mixture of $\wt{O}(k)$ Gaussians.

\begin{corollary}\label{coro:gmm-hypothesis-test}
Let $k, \eps >0$ be parameters we are given.  Let $\mcl{F}_1$ be the family of distributions that are $\eps$-close to a GMM with $k$ components (in TV distance).   Let $\mcl{F}_2$ be the family of distributions that are not $\wt{O}(\eps)$-close to any GMM with $\wt{O}(k)$ components.  There is an algorithm that given $\poly(k /\eps)$ samples from a known distribution $\mcl{D}$, runs in $\poly(k /\eps)$ time, and outputs $1$ if $\mcl{D} \in \mcl{F}_1$ and outputs $2$ if $\mcl{D} \in \mcl{F}_2$ both with failure probability at most $0.2$.
\end{corollary}
\begin{remark}
Even if the distribution $\mcl{D}$ is completely unknown and we are only given samples from it, the above result still holds as long as $\mcl{D}$ is somewhat well behaved (note that such an assumption is necessary as hypothesis testing with respect to total variation distance without any assumptions on $\mcl{D}$ is impossible).  In particular we can use piecewise polynomial approximation \cite{chan2013efficient} or kernel density estimates \cite{terrell1992variable} to learn a distribution $\mcl{D}'$ that is close to $\mcl{D}$ that we have an explicit form for and then run the hypothesis test using $\mcl{D}'$.
\end{remark}



%These formulations are particularly appropriate within scientific domains. For example, Chen et al. \cite{chen2004testing} offer as a motivation the problem of deciding how many factors control a measurable physical trait. In many situations it is unclear whether the trait is simple \--- e.g. it is monogenic, or there are just a few genes affecting it \--- or it is complex \--- i.e. it is polygenic and there are many genes that each have a small influence. In these settings the more relevant problem is not just to learn any mixture model that fits the data but to be able to approximately decide which scenario we are in, particularly in a robust way that is tolerant to model misspecification. 

The natural open question in our work is to improve our sparsity bounds, both for interpolation/learning and model selection. In principle it could be possible that there are efficient algorithms for these problems, however it is starting to seem less and less likely. Even without noise, learning a Gaussian mixture model with $k$ components without a separation condition in time $\mbox{poly}(k, 1/\epsilon)$ is open. From our work, we see that even in the well-conditioned case this is equivalent to being able to solve a structured system of polynomial equations with $O(k)$ variables representing the parameters of the mixture and $O(\log 1/\epsilon)$ constraints representing the moments. In fact, we conjecture that both the learning and model selection problems are computationally hard if we are not allowed to relax the number of components. 

\input{related_work.tex}

==> well-conditioned-cases.tex <==
%\section{The Well-Conditioned Case: GMMs}\label{sec:well-conditioned-GMMs}

%In this section, we deal with the well-conditioned case for learning GMMs. 




